A New Method for the Analysis of Signals: The Square Wave Transform (SWT)

The results obtained by analyzing signals with the Square Wave Method (SWM) introduced previously can be presented in the frequency domain clearly and precisely by using the Square Wave Transform (SWT) described here. As an example, the SWT is used to analyze a sequence of samples (that is, of measured values) taken from an electroencephalographic recording.

==> volnum.tex <==
2015 {\bf XX} (1)
